High-Capacity Urban Terrestrial Free-Space Optical Communication Links at km-Scale

Free-space optical communication links can enable high-capacity wireless connectivity in urban areas. We discuss the feasibility, challenges, and recent developments for high-capacity urban free-space optical links at kilometer scale.

==> style/includes.tex <==
%% Personal
\usepackage[utf8]{inputenc}
\usepackage{glossaries}
\usepackage[USenglish]{babel}

\newcommand{\SetCapsType}{normalcaps}
\input{acronyms.tex} %acronyms file
\usepackage[capitalise]{cleveref}
\usepackage{xcolor}
\usepackage{textgreek}
\usepackage{caption}
\usepackage{subcaption}
\usepackage[shortcuts]{extdash}
% \usepackage[adobesc, osf]{newtxtext}
% \usepackage[]{newtxmath}
\AtEndPreamble{\DeclareSymbolFont{operators}{OT1}{\rmdefault}{m}{n}}


\usepackage[per-mode=symbol]{siunitx}
\sisetup{group-separator = {,}}
\sisetup{list-final-separator = {, and }}
\DeclareSIUnit{\sample}{Sa}
\DeclareSIUnit{\baud}{Bd}
\DeclareSIUnit{\bit}{bit}
\DeclareSIUnit{\fourd}{4D}
\DeclareSIUnit{\eightd}{8D}
\DeclareSIUnit{\dBm}{dBm}
\DeclareSIUnit{\bps}{bps}

\newcommand{\cb}[1]{\textcolor{cyan}{{#1}}}
\hyphenpenalty=9999
